AutomaTikZ: Text-Guided Synthesis of Scientific Vector Graphics with TikZ

Generating bitmap graphics from text has gained considerable attention, yet for scientific figures, vector graphics are often preferred. Given that vector graphics are typically encoded using low-level graphics primitives, generating them directly is difficult. To address this, we propose the use of TikZ, a well-known abstract graphics language that can be compiled to vector graphics, as an intermediate representation of scientific figures. TikZ offers human-oriented, high-level commands, thereby facilitating conditional language modeling with any large language model. To this end, we introduce DaTikZ, the first large-scale TikZ dataset consisting of 120k TikZ drawings aligned with captions. We fine-tune LLaMA on DaTikZ, as well as our new model CLiMA, which augments LLaMA with multimodal CLIP embeddings. In both human and automatic evaluation, CLiMA and LLaMA outperform commercial GPT-4 and Claude 2 in terms of similarity to human-created figures, with CLiMA additionally improving text-image alignment. Our detailed analysis shows that all models generalize well and are not susceptible to memorization. GPT-4 and Claude 2, however, tend to generate more simplistic figures compared to both humans and our models. We make our framework, AutomaTikZ, along with model weights and datasets, publicly available.

==> figures/clima/barchart.tex <==
\begin{tikzpicture}
   \begin{axis}[
       ybar,
       ylabel={BLEU},
       ymax=43,
       symbolic x coords={Orion,Nebula,Pulsar},
       xtick=data,
       legend style={at={(0.5,-0.2)},
           anchor=north,legend columns=-1,fill=none},
       nodes near coords,
       nodes near coords align={vertical},
       every node near coord/.append style={font=\tiny},
       width=11cm,
       height=7.5cm,
       ]
       \addplot coordinates {(Orion, 38.27) (Nebula, 29.53) (Pulsar, 23.13)};
       \addplot coordinates {(Orion, 35.55) (Nebula, 26.06) (Pulsar, 21.12)};
       \addplot coordinates {(Orion, 35.99) (Nebula, 25.67) (Pulsar, 19.65)};
       \legend{Alpha, Beta, Gamma}
   \end{axis}
\end{tikzpicture}


==> figures/clima/contour.tex <==
\begin{tikzpicture}
 \begin{axis}[samples=10,domain=-3:3,y domain=-3:3]
   \addplot3 [surf] {((x)^2+(y)^2)^2};
 \end{axis}
\end{tikzpicture}


==> figures/clima/mlp.tex <==
\def\layersep{2.5cm}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep,transform shape]
   \tikzstyle{every pin edge}=[<-,shorten <=1pt]
   \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
   \tikzstyle{input neuron}=[neuron, fill=green!50]
   \tikzstyle{output neuron}=[neuron, fill=red!50]
   \tikzstyle{hidden neuron}=[neuron, fill=blue!50]
   \tikzstyle{annot} = [text width=4em, text centered]

   % Draw the input layer nodes
   \foreach \name / \y in {1,...,4}
   % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
       \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};

   % Draw the hidden layer nodes
   \foreach \name / \y in {1,...,5}
       \path[yshift=0.5cm]
           node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};

   % Draw the output layer node
   \node[output neuron,pin={[pin edge={->}]right:Output}, right of=H-3] (O) {};

   % Connect every node in the input layer with every node in the
   % hidden layer.
   \foreach \source in {1,...,4}
       \foreach \dest in {1,...,5}
           \path (I-\source) edge (H-\dest);

   % Connect every node in the hidden layer with the output layer
   \foreach \source in {1,...,5}
       \path (H-\source) edge (O);

   % Annotate the layers
   \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
   \node[annot,left of=hl] {Input layer};
   \node[annot,right of=hl] {Output layer};
\end{tikzpicture}


==> figures/examples/bad/clima-13b.tex <==
%https://arxiv.org/abs/2302.09161
\ifdefined\getCaption%
For the $P=2$ scheme, the regular cell footprint is a standard five-point
Laplacian, and if any point in the footprint is a cut cell, it is then
\enquote{irregular.} Cut cells are shown with dark shading, irregular cells with
light shading, and the remaining white cells are \enquote{regular.}
\else
\usetikzlibrary{arrows}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm, scale=1.65]
\fill[fill=black,fill opacity=0.84] (0,0) -- (2,0) -- (2,2) -- (0,2) -- cycle;
\fill[fill=black,fill opacity=0.4] (0,1) -- (2,1) -- (2,2) -- (1,2) -- cycle;
\fill[fill=black,fill opacity=0.25] (1,1) -- (2,1) -- (2,2) -- (1,2) -- cycle;
\draw (0,1)-- (2,1);
\draw (1,2)-- (2,2);
\draw (0,0)-- (2,0);
\draw (1,1)-- (2,1);
\draw (1,2)-- (2,2);
\draw (0,0)-- (0,1);
\draw (1,0)-- (1,1);
\draw (2,0)-- (2,2);
\draw (1,2)-- (1,1);
\draw [line width=1.65pt] (1,0) -- (1,1);
\draw [line width=1.65pt] (1,0) -- (2,0);
\draw [line width=1.65pt] (1,0) -- (2,1);
\draw [line width=1.65pt] (1,0) -- (2,2);
\draw [line width=1.65pt] (1,1) -- (2,1);
\draw [line width=1.65pt] (1,1) -- (1,2);
\draw [line width=1.65pt] (1,1) -- (2,2);
\draw [line width=1.65pt] (1,1) -- (2,0);
\draw [line width=1.65pt] (1,1) -- (2,1);
\draw [line width=1.65pt] (1,2) -- (2,2);
\draw [line width=1.65pt] (1,2) -- (1,1);
\draw [line width=1.65pt] (1,2) -- (2,1);
\draw [line width=1.65pt] (1,2) -- (2,0);
\draw [line width=1.65pt] (1,2) -- (2,2);
\draw [line width=1.65pt] (2,0) -- (2,1);
\draw [line width=1.65pt] (2,0) -- (1,2);
\draw [line width=1.65pt] (2,0) -- (2,2);
\draw [line width=1.65pt] (2,0) -- (2,1);
\draw [line width=1.65pt] (2,1) -- (1,2);
\draw [line width=1.65pt] (2,1) -- (2,0);
\draw [line width=1.65pt] (2,1) -- (2,2);
\draw [line width=1.65pt] (2,2) -- (1,2);
\draw [line width=1.65pt] (2,2) -- (2,1);
\draw [line width=1.65pt] (2,2) -- (1,2);
\end{tikzpicture}
\fi


==> figures/examples/bad/gpt-4.tex <==
%https://arxiv.org/abs/2304.03401
\ifdefined\getCaption%
Average Relative loss in bi-encoder recall accuracy on NQ by recall set size
depth on the baseline, Pretrained Alignment (PT), Data Augmentation (DA), and
Contrastive Alignment Post Training (CAPOT) on noisy queries.
\else
\begin{tikzpicture}
\begin{axis}[
    title={Average Relative loss in bi-encoder recall accuracy on NQ by recall set size depth},
    xmin=0, ymin=0, xmax=1, ymax=1, % Author note: added to fix warning
    axis background/.style={fill=white}, % Author note: added to preserve bg color
    xlabel={Recall set size depth},
    ylabel={Average Relative loss},
    legend pos= north east,
    ymajorgrids=true,
    grid style=dashed,
]
% Author note: Commented out to fix compile errors
%\addplot[color=blue, mark=square] table {data1.dat}; \addlegendentry{baseline}
%\addplot[color=red, mark=triangle] table {data2.dat}; \addlegendentry{PT}
%\addplot[color=brown, mark=x] table {data3.dat}; \addlegendentry{DA}
%\addplot[color=green, mark=star] table {data4.dat}; \addlegendentry{CAPOT}
\end{axis}
\end{tikzpicture}
\fi


==> figures/examples/bad/llama-13b.tex <==
%https://arxiv.org/abs/2106.10863
\ifdefined\getCaption%
Illustration of the proof of Theorem 2.7. \emph{The image displays a tree with
blue and orange labels on a white background. The tree has a unique structure,
with branches that don't follow a typical tree layout. The labels seem to be
representing a formula or a set of instructions, and the tree is accompanied by
several equations in the surrounding area.}
\else
\begin{tikzpicture}
\draw (0,0) node[draw=black, fill=blue!30, circle, inner sep=0pt, minimum size=5pt] (l') {};
\draw (0,-1) node[draw=black, fill=orange!70, circle, inner sep=0pt, minimum size=5pt] (l) {};
\draw (-1,-2) node[draw=black, fill=orange!70, circle, inner sep=0pt, minimum size=5pt] (ll) {};
\draw (1,-2) node[draw=black, fill=orange!70, circle, inner sep=0pt, minimum size=5pt] (lr) {};
\draw (l') -- (ll) -- (l) % Author note: removed inexistent node to fix error
	(l') -- (l)
	(ll) -- (lr)
	(l') -- (lr);
\draw (ll) -- ++(-30:0.5cm)	node[shift={(-0.2,-0.2)}] {\scriptsize $R_2$};
\draw (lr) -- ++(30:0.5cm)	node[shift={(-0.1,-0.1)}] {\scriptsize $R_2$};
\draw (l') ++(-30:0.25cm) -- ++(-30:0.5cm)	node[shift={(-0.1,-0.1)}] {\scriptsize $R_1$};
\draw (l') ++(30:0.25cm) -- ++(30:0.5cm)	node[shift={(-0.2,-0.2)}] {\scriptsize $R_1$};
\draw (l) ++(150:0.25cm) -- ++(150:0.5cm)	node[left,xshift=0.2cm,yshift=-0.2cm] {\scriptsize $R_3$};
\draw (l) ++(-150:0.25cm) -- ++(-150:0.5cm)	node[left, xshift=0.1cm, yshift=0.1cm] {\scriptsize $R_3$};
\node at (0, 0.5) {\scriptsize $l$};
\node at (0, -1.5) {\scriptsize $l'$};
\node at (-1.5, -2.5) {\scriptsize $l_1$};
\node at (1.5, -2.5) {\scriptsize $l_2$};
\end{tikzpicture}
\fi


==> figures/examples/good/clima-13b.tex <==
%https://arxiv.org/abs/2304.12339
\ifdefined\getCaption%
The ansatz (5.17) and (5.18) for $\alpha=2$. The red points are evenly spaced,
and the blue points scale quadratically with $n$.\ \emph{The image is a white
background with blue and red dots scattered across it. The dots are placed in
various arrangements, creating a visually interesting pattern. Some dots are
clustered together, while others are spaced further apart, covering the entire
background.}
\else
\begin{tikzpicture}
    \draw (0,0) -- (10,0);
    \foreach \x in {0,1,...,10} {\draw (\x,-.1) -- (\x,.1);}
    \foreach \x in {0,1,...,10} \foreach \y in {0,1,...,4} {\fill[red] (\x,\y) circle (0.05);}
    \foreach \x in {0,1,...,10} \foreach \y in {1,2,..., 4} {\fill[blue] (\x,{\y/2}) circle (0.05);}
    \foreach \x in {0,1,...,10} \foreach \y in {1,2,..., 4} {\fill[blue] (\x,{4-\y/2}) circle (0.05);}
    \foreach \y in {1,2,..., 4} {\fill[blue] (5, \y) circle (0.05);}
    \foreach \y in {1,2,..., 4} {\fill[blue] (5, 4-\y) circle (0.05);}
    \draw (5,.1) -- (5,-.1);
    \node[below] at (5,-.1) {$n$};

    \begin{scope}[yshift=-2.25cm]
    \draw (0,0) -- (10,0);
    \foreach \x in {0,1,...,10} {\draw (\x,-.1) -- (\x,.1);}
    \foreach \x in {0,1,...,10} \foreach \y in {0,1,...,4} {\fill[red] (\x,\y) circle (0.05);}
    \foreach \x in {0,1,...,10} \foreach \y in {1,2,..., 4} {\fill[blue] (\x,{\y/2}) circle (0.05);}
    \foreach \x in {0,1,...,10} \foreach \y in {1,2,..., 4} {\fill[blue] (\x,{4-\y/2}) circle (0.05);}
    \foreach \y in {1,2,..., 4} {\fill[blue] (5, \y) circle (0.05);}
    \foreach \y in {1,2,..., 4} {\fill[blue] (5, 4-\y) circle (0.05);}
    \draw (5,.1) -- (5,-.1);
    \node[below] at (5,-.1) {$2n$};
    \end{scope}
\end{tikzpicture}
\fi


==> figures/examples/good/gpt-4.tex <==
%https://arxiv.org/abs/2301.00587
\ifdefined\getCaption%
Expression graph for algebraic expression $x^2 + 2xy+y^2$.\ \emph{The image
shows a tree with a symbol at its root, representing a mathematical concept.
The tree has a series of logical connections, and there are variables and
mathematical symbols throughout the structure. The image conveys a sense of
order and organization in the presentation of the mathematical concept.}
\else
\usetikzlibrary{trees}
\begin{tikzpicture}[
  every node/.style = {shape=circle, draw},
  level 1/.style = {sibling distance=4cm, level distance=1.5cm},
  level 2/.style = {sibling distance=2cm},
  level 3/.style = {sibling distance=1cm}
]
\node {+}
  child {node {(x)²}
    child{node{x}
      child{node{x}}
    }
  }
  child {node {+}
    child {node {2xy}
      child{node{2}}
      child{node{x}}
      child{node{y}}
    }
    child{node{(y)²}
      child{node{y}
        child{node{y}}
      }
    }
  };
\end{tikzpicture}
\fi


==> figures/examples/good/llama-13b.tex <==
%https://arxiv.org/abs/2305.05755
\ifdefined\getCaption%
Local configuration of the path and the foliation (in red) around the point
$0=\Psi_z(z)$.\ \emph{The image displays a complex mathematical formula with
various symbols and notation, including a black dot, waves, and arrows. The
formula seems to be related to physics or engineering, and it is written on a
white background for easy readability.}
\else
\begin{tikzpicture}
\draw[red] (0,0).. controls (1,-1) and (1.5,-0.5)..(2,0);
\draw[red] (0,0).. controls (1,1) and (1.5,0.5)..(2,0);
\draw[thick] (1,-1.5)--(1,1.5);
\draw[thick, dashed, ->] (1.2,0.8)--(1.5,0.7);
\draw[thick, dashed, ->] (1,0)--(1.3,0.2);
\draw[thick, dashed] (1.5,0.7)--(2,0.7);
\draw[thick, dashed] (1.3,0.2)--(2,0.2);
\draw[thick, dashed, ->] (1.2,-0.8)--(1.5,-0.7);
\draw[thick, dashed, ->] (1,-0.5)--(1.3,-0.3);
\draw[thick, dashed] (1.5,-0.7)--(2,-0.7);
\draw[thick, dashed] (1.3,-0.3)--(2,-0.3);
\draw (2.2,0) node[right]{$T_z \mathcal P$};
\draw (0,0) node{$\bullet$};
\draw (0,0) node[below left]{$0=\zeta_z(z)$};
\draw[thick, dashed,->] (1.4,0.94) to[out=200, in=80] (0,0);
\draw[thick, dashed,->] (1.4,-0.94) to[out=340, in=260] (0,0);
\draw (1.5,1) node[above]{$\mathcal L_{\gamma_z(z)}$};
\end{tikzpicture}
\fi


==> latexmkrc <==
use File::Spec::Functions 'catfile';
use Cwd 'abs_path';
use File::Basename;
use File::Find;

## General configuration
# -----------------------------------------------------------------------------
$out_dir = "build";
$pdf_mode = 1;
$bibtex_use = 1.5;
$cleanup_includes_cusdep_generated = 1;
$cleanup_includes_generated = 1;
$pre_tex_code = "\\PassOptionsToPackage{outputdir=$out_dir}{minted}";

ensure_path('TEXINPUTS', abs_path('styles'));
ensure_path('BSTINPUTS', abs_path('styles'));

## Custom dependencies
# -----------------------------------------------------------------------------
my $figures_out_dir = "$out_dir/figures/";
my @figures = ('figures/', glob('figures/*/'));

# generate plots with python (through seaborn)
add_cus_dep('py', 'pdf', 0, 'seaborn');
sub seaborn {
  my $module = join(".", split("/", substr($$Psource, 0, -3)));
  $$Pdest = catfile($figures_out_dir, basename($$Pdest));

  # add all data files to list of source files for this rule
  # this could be improved by adding only data files which are actually used
  find({
      wanted => sub {if ( !-d ) { rdb_ensure_file($rule, $_) }},
      no_chdir => 1
    },
    catfile(dirname($$Psource), "data")
  );

  return Run_subst("python -m %S %D", 1, "", $module);
}

# make sure that latex finds all of these files
ensure_path('TEXINPUTS', @figures, $figures_out_dir);

# https://tex.stackexchange.com/a/40924
set_tex_cmds('--interaction=nonstopmode --shell-escape %O %P');

# vim: filetype=perl

